Online 3D Bin Packing with Constrained Deep Reinforcement Learning

We solve a challenging yet practically useful variant of 3D Bin Packing Problem (3D-BPP). In our problem, the agent has limited information about the items to be packed into the bin, and an item must be packed immediately after its arrival without buffering or readjusting. The item's placement also subjects to the constraints of collision avoidance and physical stability. We formulate this online 3D-BPP as a constrained Markov decision process. To solve the problem, we propose an effective and easy-to-implement constrained deep reinforcement learning (DRL) method under the actor-critic framework. In particular, we introduce a feasibility predictor to predict the feasibility mask for the placement actions and use it to modulate the action probabilities output by the actor during training. Such supervisions and transformations to DRL facilitate the agent to learn feasible policies efficiently. Our method can also be generalized e.g., with the ability to handle lookahead or items with different orientations. We have conducted extensive evaluation showing that the learned policy significantly outperforms the state-of-the-art methods. A user study suggests that our method attains a human-level performance.

==> broader.tex <==
\section*{Broader Impact}\label{sec:borader}
%\setlength{\columnsep}{10 pt}
%\begin{wrapfigure}{r}{0.40\linewidth}
%\vspace{-20 pt}
%	\includegraphics[width = \linewidth]{fig/teaser.pdf}
%    \vspace{-15 pt}
%	\caption*{3D-BPP is widely useful in logistics, manufacture, warehousing etc.}\label{fig:teaser}
%\vspace{-10 pt}
%\end{wrapfigure}
We believe the broader impact of this research is significant. BPP is considered as the one of the most needed academic problems due to its wide applicability in our daily lives~\cite{skiena1997stony}. Providing a good solution to 3D-BPP yields direct and profound impacts beyond academia. A practical application scenario of our algorithm is illustrated in Figure.~\ref{fig:teaser}. The conveyor belt sends a sequence of items to a robot agent. Those items are scanned by an overhead depth sensor, so that the information of their dimensions can be obtained using some basic computer vision technique. The agent places the item as soon as it arrives. We note that such setup has been already widely deployed in logistics hubs and manufacture plants. A good BPP solution benefits all the downstream operations like package wrapping, transportation, warehousing and distribution.

Aside from its real-world applications, 3D-BPP algorithm proposed in this paper is generalizable and transformative. As a member of NP-Hard family, an algorithm to 3D-BPP can be reduced to a solution to many other difficult NP-Hard problems including the famous knapsack problem, dominating set problem, nurse scheduling problem, or cut socking problem. Our constrained DRL framework and its novel solution has a good potential for solving a wide category of combinatorial problems.

